Towards Composable Concurrency Abstractions

In the past decades, many different programming models for managing concurrency in applications have been proposed, such as the actor model, Communicating Sequential Processes, and Software Transactional Memory. The ubiquity of multi-core processors has made harnessing concurrency even more important. We observe that modern languages, such as Scala, Clojure, or F#, provide not one, but multiple concurrency models that help developers manage concurrency. Large end-user applications are rarely built using just a single concurrency model. Programmers need to manage a responsive UI, deal with file or network I/O, asynchronous workflows, and shared resources. Different concurrency models facilitate different requirements. This raises the issue of how these concurrency models interact, and whether they are composable. After all, combining different concurrency models may lead to subtle bugs or inconsistencies. In this paper, we perform an in-depth study of the concurrency abstractions provided by the Clojure language. We study all pairwise combinations of the abstractions, noting which ones compose without issues, and which do not. We make an attempt to abstract from the specifics of Clojure, identifying the general properties of concurrency models that facilitate or hinder composition.

==> eptcsdata.tex <==
\providecommand{\firstpage}{54}
\providecommand{\publicationstatus}{Alastair F. Donaldson, Vasco Vasconcelos (Eds.): Proceedings\\ of the 7th Workshop on Programming Language Approaches\\ to Concurrency and Communication-cEntric Software (PLACES 2014)\\
EPTCS 155, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.155.8}{10.4204/EPTCS.155.8}}

